Is Context Helpful for Chat Translation Evaluation?

Despite the recent success of automatic metrics for assessing translation quality, their application in evaluating the quality of machine-translated chats has been limited. Unlike more structured texts like news, chat conversations are often unstructured, short, and heavily reliant on contextual information. This poses questions about the reliability of existing sentence-level metrics in this domain as well as the role of context in assessing the translation quality. Motivated by this, we conduct a meta-evaluation of existing sentence-level automatic metrics, primarily designed for structured domains such as news, to assess the quality of machine-translated chats. We find that reference-free metrics lag behind reference-based ones, especially when evaluating translation quality in out-of-English settings. We then investigate how incorporating conversational contextual information in these metrics affects their performance. Our findings show that augmenting neural learned metrics with contextual information helps improve correlation with human judgments in the reference-free scenario and when evaluating translations in out-of-English settings. Finally, we propose a new evaluation metric, Context-MQM, that utilizes bilingual context with a large language model (LLM) and further validate that adding context helps even for LLM-based evaluation metrics.

==> figs/prompt_no_context.tex <==
  \begin{figure*}[htb!]
         \renewcommand\tabularxcolumn[1]{m{#1}}% <-- added
        \renewcommand\arraystretch{1.2}
    \begin{tabularx}{\linewidth}{*{1}{>{\arraybackslash}X}}
  \textbf{System:}  You are an annotator for the quality of machine translation. Your task is to identify errors and assess the quality of the translation. \\
  The categories of errors are: accuracy (addition, mistranslation, omission, untranslated text), fluency (character encoding, grammar, inconsistency, punctuation, register, spelling), style (awkward), terminology (inappropriate for context, inconsistent use), non-translation, other, source error or no-error.\\
  Each error is classified as one of three categories: critical, major, and minor. Critical errors inhibit comprehension of the text. Major errors disrupt the flow, but what the text is trying to say is still understandable. Minor errors are technically errors, but do not disrupt the flow or hinder comprehension.\\
  \textbf{User}: English source:\\
  ```As soon as we have heard back, tis is when you will be emailed``` \\
  German translation:\\
  ```Sobald wir wieder gehört haben, tis ist, wenn Sie e-mail erhalten werden``` \\
  
  Based on the source segment and machine translation surrounded with triple backticks, identify error types in the translation and classify them.

  \textbf{Assistant}: 'Critical: \\
  accuracy/untranslated -"tis" \\
  Major:\\
  accuracy/mistranslation - "wieder gehört haben" \\
  Minor: \\
  accuracy/addition - "wenn"\\
  source issue - "tis"\\
   
   \textbf{User}: English source:
   ```As we do not carry stock then all items are made to order, shipped on to us here at #URL# and then sent onto yourselves.```\\
   German translation:\\
   ```Da wir keine Lager führen, werden alle Artikel auf Bestellung gefertigt, an uns hier bei #URL# gesendet und dann an Sie gesendet.```\\
   
   Based on the source segment and machine translation surrounded with triple backticks, identify error types in the translation and classify them.
    \end{tabularx}  
\caption{ Prompt (No Context) } \label{fig:prompt}
\end{figure*}


==> tables/data_tmp.tex <==


  \pgfplotstableread{ % data 
Label     weak moderate good excellent
EnDe   3.53 3.57 4.77 88.12
    }\ende

  \pgfplotstableread{ % data 
Label     weak moderate good excellent
DeEn 4.64 3.61 6.82 84.92 
    }\deen
  \pgfplotstableread{ % data 
Label     weak moderate good excellent
EnPt   
    }\enpt
  \pgfplotstableread{ % data 
Label     weak moderate good excellent
PtEn  
    }\pten
  \pgfplotstableread{ % data 
Label     weak moderate good excellent
EnFr   
    }\enfr
  \pgfplotstableread{ % data 
Label     weak moderate good excellent
FrEn  
    }\freen

\pgfplotsset{compat=1.17}


\begin{table*}[ht]
\centering
 \setlength\tabcolsep{2.4pt}
\scalebox{0.75}{
\begin{tabular}{lcccrrrrrp{3cm}r}
 \toprule
  % \rowcolor{gray!10}
 & \multicolumn{3}{c}{\textsc{\textbf{Count}}} & \multicolumn{3}{c}{\textsc{\textbf{Length}}} & &   \\
 % \rowcolor{gray!40}
\textsc{\textbf{LP}} & \# (Instances) & \# (Conversations) & \# (Systems) & Source & MT & Ref &\multicolumn{1}{c} {\textbf{CUA}} & \% Perfect MQM\\
\midrule
en-de (Agent) & 2715 & 30 & 5 & 48.82 & 57.34 & 57.20 &     \begin{tikzpicture}
    \begin{axis}[
    hide x axis,
    hide y axis,
    xbar stacked,   % Stacked horizontal bars
    xmin=0,         % Start x axis at 0
    ytick=data,     % Use as many tick labels as y 
    width=5cm,      % Set the width of the plot
    height=4cm,     % Set the height of the plot
    ]
    \addplot [fill=red!80] table [x=weak, meta=Label,y expr=\coordindex] {\ende};   % "First" column against the data index
    \addplot [fill=red!20] table [x=moderate, meta=Label,y expr=\coordindex] {\ende};
    \addplot [fill=green!20] table [x=good, meta=Label,y expr=\coordindex] {\ende};
    \addplot [fill=green!80] table [x=excellent, meta=Label,y expr=\coordindex] {\ende};
    \end{axis}
    \end{tikzpicture} & 73.6 \\
de-en (Client) & 2720 &  &  & 38.14 & 34.46 & 35.49 & \begin{tikzpicture}
    \begin{axis}[
    hide x axis,
    hide y axis,
    xbar stacked,   % Stacked horizontal bars
    xmin=0,         % Start x axis at 0
    ytick=data,     % Use as many tick labels as y 
    width=5cm,      % Set the width of the plot
    height=4cm,     % Set the height of the plot
    ]
    \addplot [fill=red!80] table [x=weak, meta=Label,y expr=\coordindex] {\deen};   % "First" column against the data index
    \addplot [fill=red!20] table [x=moderate, meta=Label,y expr=\coordindex] {\deen};
    \addplot [fill=green!20] table [x=good, meta=Label,y expr=\coordindex] {\deen};
    \addplot [fill=green!80] table [x=excellent, meta=Label,y expr=\coordindex] {\deen};
    \end{axis}
    \end{tikzpicture} & 65.4 \\
% en-fr (Agent) & 1868 & 23 & 2 & 36.26 & 42.81 & 44.21 & 100 & 118 & 129 & 1274 & 46.7\\
% fr-en (Client) & 1020 & & & 35.72 & 32.36 & 3319 & 45 & 37 & 41 & 748 & 65.7 \\
% en-pt (Agent) & 1318 & 28 & 2 & 43.21 & 46.34 & 45.96 & 77 & 81 & 103 & 872 & 50.1 \\
% pt-en (Client) & 1016 & & & 30.44 & 31.06 & 3135 & 40 & 68 & 66 & 624 & 54.5 \\
% \midrule
% Total &  10657 & 81 && 9 &  \\
  \bottomrule
 \end{tabular}
 }
\caption{Data Statistics \sa{convert CUA into bars with percentages according to the colors; receheck source issues and whether to include them ; need to update}}\label{tab:data_stats} 
\end{table*}



==> unbabel_mqm/benchmark.tex <==

% into-en
\begin{table*}[ht]
\centering
 % \setlength\tabcolsep{2pt}
\scalebox{0.85}{
\begin{tabular}{lrrrrrrrr}
 \toprule
 \multirow{2}{*}{\textsc{\textbf{Metric}}} & \multicolumn{2}{c}{\textsc{\textbf{Average}}}  & \multicolumn{2}{c}{\textsc{\textbf{De-En}}} & \multicolumn{2}{c}{\textsc{\textbf{Fr-En}}} & \multicolumn{2}{c}{\textsc{\textbf{Pt-En}}} \\
 & All & All-100MQM  & All & All-100MQM  & All & All-100MQM  & All & All-100MQM  \\
\midrule
chrF &  0.446 &	0.378 &	0.413 &	0.361 &	0.429 &	0.354 &	0.495	& 0.418\\
BLEU &  0.407 &	0.285	 &0.402 &	0.304 &	0.381 &	0.238 &	0.438 &	0.313\\

\addlinespace[0.2cm]

BERTScore & 0.493 &	0.391 &	0.451 &	0.360 &	0.466 &	0.363 &	0.563 &	0.450\\
Prism (NLLB) & 0.403 &	\textbf{0.495} &	0.347 &	\textbf{0.436} &	0.372	 &\textbf{0.511} &0.489 &	\textbf{0.539}\\
BLEURT & 0.541 &	0.431 &	0.499 &	0.372 &	0.537	 &0.466 &	0.587 &	0.455\\
Comet22 & \textbf{0.584} &	0.372 &	\textbf{0.564} &	0.330	 &\textbf{0.567}	 &0.372 &	\textbf{0.620} &	0.414 \\
% xCOMET-XL & 0.418	& 0.320 & 0.336 &	0.332	& 0.454 &	0.328 &	0.465 &	0.299 \\

\addlinespace[0.2cm]

Comet20-QE & 0.474 &	0.189	&0.533	&0.240 &	0.438 &	0.177 &	0.452	& 0.151\\
Comet22-QE & 0.424 &	0.378 &	0.370 &	0.377 &	0.453 &	0.398 &	0.448 &	0.359 \\
% CometKIWI-XL & 0.223&	0.350&	0.111&	0.374	&0.281	&0.339&	0.278&	0.337\\
% xCOMET-XL  (QE) & 0.409&	0.235	&0.354 &	0.224	&0.434	&0.238&	0.439&	0.242 \\
  \bottomrule
 \end{tabular}
 }
\caption{Benchmark (Customer)}\label{tab:benchmarkintoeng} 
\end{table*}
% does comet penalize formality

% outof-en
\begin{table*}[ht]
\centering
 % \setlength\tabcolsep{2pt}
\scalebox{0.85}{
\begin{tabular}{lrrrrrrrr}
 \toprule
 \multirow{2}{*}{\textsc{\textbf{Metric}}} & \multicolumn{2}{c}{\textsc{\textbf{Average}}}  & \multicolumn{2}{c}{\textsc{\textbf{En-De}}} & \multicolumn{2}{c}{\textsc{\textbf{En-Fr}}} & \multicolumn{2}{c}{\textsc{\textbf{En-Pt}}} \\
 & All & All-100MQM  & All & All-100MQM  & All & All-100MQM  & All & All-100MQM  \\
\midrule
chrF & 0.535 &	0.525 &	0.434 &	0.442 &	0.692 &	0.663 &	0.479 &	0.469\\
BLEU & 0.502 &	0.401 &	0.364 &	0.262 &	0.663 &	0.542 &	0.478 &	0.400\\

\addlinespace[0.2cm]

BERTScore & 0.549 &	0.501 &	0.442 &	0.418 &	\textbf{0.703} &	0.627 &	0.501	 &0.459\\
Prism (NLLB) & 0.252 &	\textbf{0.627} &	0.253 &	\textbf{0.507} &	0.175 &	\textbf{0.750} &	0.328 &	\textbf{0.625}\\
BLEURT &0.511 &	0.513 &	0.427 &	0.467 &	0.639 &	0.647 &	0.468 &	0.424\\
Comet22 & \textbf{0.592} &	0.399 &	\textbf{0.560} &	0.310 &	0.698 &	0.558 &	\textbf{0.518} &	0.329 \\
% xCOMET-XL & 0.334 &	0.209	&0.369 &	0.072 &	0.319 &	0.426 &	0.314 &	0.129\\

\addlinespace[0.2cm]

Comet20-QE & 0.302 &	0.052	&0.383	&0.081&	0.293&	0.092	&0.231 &	-0.018\\
Comet22-QE & 0.300 &	0.393 &	0.364	 &0.377 &	0.218 &	0.549 &	0.319 &	0.254 \\
% CometKIWI-XL & 0.222&	0.357&	0.272&	0.266	&0.138	&0.493&	0.256 &	0.311\\
% xCOMET-XL (QE) & 0.187 &	-0.007	&0.313 &	0.018	&0.060	&0.057	&0.187	&-0.096\\
  \bottomrule
 \end{tabular}
 }
\caption{Benchmark (Agent)}\label{tab:benchmarkoutofeng} 
\end{table*}




% \begin{enumerate}
%     \item \textbf{BLEU} \cite{papineni2002bleu} estimates the translation quality based on n-gram overlap between the hypotheses and references. We compute sentence-level BLEU \cite{chen-cherry-2014-systematic}  between the hypothesis and the reference using the \textsc{Sacrebleu} library.\footnote{\url{https://github.com/mjpost/sacrebleu/}: nrefs:1$\vert$case:mixed$\vert$eff:no$\vert$tok:13a$\vert$smooth:exp$\vert$version:2.4.0}
%     \item \textbf{\textsc{chrF}} \cite{popovic2015chrf} evaluates the similarity by computing an F1 score between the overlapping character n-grams in the candidate and reference translations.
%     \item \textbf{\textsc{BERTScore}} \cite{zhang2019bertscore} uses the cosine similarity between the pre-trained contextualized embeddings to measure the similarity between the candidate translations and the reference texts.
%     \item \textbf{BLEURT} \cite{sellam2020bleurt} utilizes pre-trained transformer models to estimate a quality score that reflects the semantic similarity between the candidate and reference texts. BLEURT is a neural regression metric trained on an existing collection of human judgments. 
%     % \item \textbf{Prism (NLLB)} \cite{thompson2020automatic} involves computing the log-likelihood of the hypothesis given the reference and vice-versa, given a multilingual MT model. We use \texttt{NLLB-200-distilled-600M} for our evaluation.
%     \item \textbf{\textsc{Comet-22}} \cite{rei-etal-2022-comet} is a XLM-R-based \cite{conneau2020unsupervised} regression model trained on direct assessments from WMT17 to WMT20 and provides scores ranging from 0 to 1. Unlike BLEURT which only utilizes the reference and the candidate texts, COMET uses the triplet (source sentence, translation, reference translation) to return a score that reflects the quality of the translation compared to both source and reference.
%     \item \textbf{\textsc{Comet-20-QE}} \cite{rei-etal-2020-unbabels} is a regression-based metric trained to predict the direct assessment scores using representations extracted from the (source, hypothesis) pair. It uses XLM-R as the base architecture.
%     \item \textbf{\textsc{CometKiwi-22-QE}} \cite{rei-etal-2022-cometkiwi} is a reference-free model built on top of the \textsc{InfoXLM-R} model \cite{chi-etal-2021-infoxlm} and is trained to predict direct assessments from WMT17-20 and the MLQE-PE corpus \cite{fomicheva-etal-2022-mlqe}. It generates scores ranging from 0 to 1. 
%      \item \textbf{\textsc{xComet-XL}} \cite{guerreiro2023xcomet}, with 3.5B parameters, is a recent state-of-the-art explainable learned metric trained to predict both sentence-level quality scores and MQM-like error spans from the (source sentence, translation, reference translation) triplet. Furthermore, the metric can also be used for quality estimation by using only the source sentence and the candidate translations as input, referred to as \textsc{xComet-QE-XL}.
%      \item \textbf{\textsc{MetricX-23-XL}} \cite{juraska-etal-2023-metricx} is a regression-based metric built on top of mT5 \cite{xue-etal-2021-mt5} and is trained to regress the true MQM score in the range [0, 25] where a lower score is better as it predicts an error score. The input to the model is the candidate (hypothesis) and reference translations—each with a corresponding prefix (``candidate:'' and ``reference:'', respectively)—concatenated together. \\
%      \item \textbf{\textsc{MetricX-23-QE-XL}} \cite{juraska-etal-2023-metricx}  is a reference-free version of \textsc{MetricX-23-XL} that takes as input the source and the candidate translation to predict a quality rating in the same range of [0, 25].  \\
% \end{enumerate}



